NLLG Quarterly arXiv Report 09/24: What are the most influential current AI Papers?

The NLLG (Natural Language Learning & Generation) arXiv reports assist in navigating the rapidly evolving landscape of NLP and AI research across cs.CL, cs.CV, cs.AI, and cs.LG categories. This fourth installment captures a transformative period in AI history - from January 1, 2023, following ChatGPT's debut, through September 30, 2024. Our analysis reveals substantial new developments in the field - with 45% of the top 40 most-cited papers being new entries since our last report eight months ago and offers insights into emerging trends and major breakthroughs, such as novel multimodal architectures, including diffusion and state space models. Natural Language Processing (NLP; cs.CL) remains the dominant main category in the list of our top-40 papers but its dominance is on the decline in favor of Computer vision (cs.CV) and general machine learning (cs.LG). This report also presents novel findings on the integration of generative AI in academic writing, documenting its increasing adoption since 2022 while revealing an intriguing pattern: top-cited papers show notably fewer markers of AI-generated content compared to random samples. Furthermore, we track the evolution of AI-associated language, identifying declining trends in previously common indicators such as "delve".

==> structure/tables/ppcount.tex <==
\begin{table}[tb]
    \begin{subtable}{1\linewidth}
      \centering
\scriptsize
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Sector}&\textbf{Sector Total} &\textbf{US} &\textbf{CN} &\textbf{Europe} &\textbf{The rest} \\\midrule
\textbf{Academia} &54.63\% &22.93\% &15.85\% &3.81\% &12.04\% \\
\textbf{Industry} &45.37\% &31.56\% &6.38\% &1.10\% &6.34\% \\
\textbf{Region \zrf{Total}}  & 100.00\% &54.49\%	& 22.23\% &	4.91\% & 18.37\% \\
\bottomrule
\end{tabular}
\caption{Top-40 papers.}
\label{tab:pptop40}
    \end{subtable}%
    \bigskip
    \\
    \begin{subtable}{1\linewidth}
      \centering
        \centering
\scriptsize
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Sector} &\textbf{Sector Total} &\textbf{US} &\textbf{CN} &\textbf{Europe} &\textbf{The rest} \\\midrule
\textbf{Academia} &92.46\% &30.61\% &25.12\% &18.38\% &18.35\% \\
\textbf{Industry} &7.54\% &5.02\% &1.63\% &	0.36\% & 0.54\% \\
\textbf{Region \zrf{Total}} &100.00\% &35.63\% &26.75\% &18.74\% &	18.89\% \\
\bottomrule
\end{tabular}
\caption{Top-8k papers.}
\label{tab:pptop9k}
    \end{subtable} 
    \caption{(a) The percentage contribution of institutional sectors and regions based on proportional count for the \arxivsmall{} papers. (b) The percentage contribution of institutional sectors and regions based on proportional count for the \topk{} papers in the \sept{} dataset.}
    \label{tab:ppcount}
\end{table}


==> structure/tables/trigram.tex <==
\begin{table}[tb]
    \centering
    \small
    %\setlength{\tabcolsep}{1pt}
    %\renewcommand{\arraystretch}{0.1}
    %\fontsize{8.5pt}{8.5pt}\selectfont
    \begin{tabular}{m{1.5cm}  m{10cm}  m{2.5cm}}
    \toprule
month & trigram & percentages \\ \midrule
2023-01 & (graph neural networks),(deep reinforcement learning),(large language models),(deep neural networks),(self supervised learning) & 1.0,0.7,0.6,0.4,0.4 \\ \midrule
2023-02 & (large language models),(graph neural networks),(deep neural networks),(deep reinforcement learning),(self supervised learning) & 0.9,0.9,0.6,0.6,0.5 \\ \midrule
2023-03 & (large language models),(graph neural networks),(self supervised learning),(3d object detection),(deep neural networks) & 1.0,0.6,0.5,0.5,0.5 \\ \midrule
2023-04 & (large language models),(medical image segmentation),(deep reinforcement learning),(deep neural networks),(self supervised learning) & 1.9,0.7,0.7,0.6,0.6 \\ \midrule
2023-05 & (large language models),(graph neural networks),(pre trained language),(deep neural networks),(large language model) & 3.5,0.7,0.5,0.5,0.5 \\ \midrule
2023-06 & (large language models),(graph neural networks),(medical image segmentation),(deep reinforcement learning),(pre trained language) & 2.4,0.7,0.6,0.5,0.4 \\ \midrule
2023-07 & (large language models),(graph neural networks),(large language model),(self supervised learning),(deep neural networks) & 2.9,0.8,0.7,0.6,0.6 \\ \midrule
2023-08 & (large language models),(large language model),(graph neural networks),(deep reinforcement learning),(deep learning based) & 3.3,0.7,0.6,0.6,0.5 \\ \midrule
2023-09 & (large language models),(large language model),(deep reinforcement learning),(deep neural networks),(graph neural networks) & 3.9,0.8,0.6,0.4,0.4 \\ \midrule
2023-10 & (large language models),(large language model),(graph neural networks),(deep reinforcement learning),(using large language) & 5.9,1.2,0.8,0.5,0.5 \\ \midrule
2023-11 & (large language models),(large language model),(graph neural networks),(vision language models),(self supervised learning) & 4.7,1.0,0.7,0.5,0.4 \\ \midrule
2023-12 & (large language models),(large language model),(graph neural networks),(deep reinforcement learning),(vision language models) & 3.7,1.0,0.6,0.6,0.4 \\ \midrule
2024-01 & (large language models),(large language model),(graph neural networks),(deep reinforcement learning),(deep learning based) & 5.3,1.5,0.7,0.5,0.4 \\ \bottomrule
\end{tabular}
\caption{Monthly top 5 trigrams in the titles and their percentages in our data.}
    \label{tab:trigram_title}
\end{table}

\begin{table}[tb]
    \centering
    \small
    %\setlength{\tabcolsep}{1pt}
    %\renewcommand{\arraystretch}{0.1}
    %\fontsize{8.5pt}{8.5pt}\selectfont
    \begin{tabular}{m{1.5cm}  m{10cm}  m{2.5cm}}
    \toprule
month & trigram & percentages \\ \midrule
2023-01 & (deep neural networks),(natural language processing),(machine learning models),(reinforcement learning rl),(deep learning based) & 3.2,2.7,2.1,2.1,2.0 \\\midrule
2023-02 & (deep neural networks),(natural language processing),(graph neural networks),(large language models),(deep learning models) & 3.6,2.9,2.3,2.2,2.0 \\\midrule
2023-03 & (deep neural networks),(large language models),(natural language processing),(deep learning models),(machine learning models) & 3.8,2.9,2.6,2.1,2.0 \\\midrule
2023-04 & (large language models),(deep neural networks),(language models llms),(natural language processing),(deep learning based) & 5.0,3.1,3.0,3.0,2.1 \\\midrule
2023-05 & (large language models),(language models llms),(natural language processing),(deep neural networks),(pre trained language) & 8.8,6.3,3.6,2.7,2.4 \\\midrule
2023-06 & (large language models),(language models llms),(natural language processing),(deep neural networks),(reinforcement learning rl) & 6.3,4.0,2.9,2.9,2.3 \\\midrule
2023-07 & (large language models),(language models llms),(natural language processing),(deep neural networks),(machine learning models) & 6.9,4.9,3.1,3.0,2.3 \\\midrule
2023-08 & (large language models),(language models llms),(natural language processing),(deep neural networks),(machine learning models) & 7.9,5.7,2.9,2.8,2.3 \\\midrule
2023-09 & (large language models),(language models llms),(deep neural networks),(natural language processing),(machine learning models) & 10.0,7.2,2.8,2.7,2.3 \\\midrule
2023-10 & (large language models),(language models llms),(natural language processing),(deep neural networks),(graph neural networks) & 14.4,11.1,3.5,2.6,2.1 \\\midrule
2023-11 & (large language models),(language models llms),(natural language processing),(deep neural networks),(machine learning models) & 12.5,9.1,2.9,2.1,2.0 \\\midrule
2023-12 & (large language models),(language models llms),(natural language processing),(deep neural networks),(reinforcement learning rl) & 10.7,7.6,2.7,2.4,1.9 \\\midrule
2024-01 & (large language models),(language models llms),(natural language processing),(deep neural networks),(graph neural networks) & 13.5,9.6,3.6,2.4,2.1 \\ \bottomrule
\end{tabular}
\caption{Monthly top 5 trigrams in the abstracts and their percentages in our data.}
    \label{tab:trigram_abstract}
\end{table}


==> tikzlibrarytimeline.code.tex <==
% * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *
% COPYRIGHT 2014 - Claudio Fiandrino
% Released under the LaTeX Project Public License v1.3c or later
% 
% email: <claudio dot fiandrino at gmail dot com>
%
% Timeline TikZ library version 0.3b - 25/02/2019

\usetikzlibrary{backgrounds,calc}

\pgfkeys{/tikz/.cd,
  timespan/.store in=\timespan,
  timespan=Week,
  timeline width/.store in=\timelinewidth,
  timeline width=20,
  timeline height/.store in=\timelineheight,
  timeline height=1,
  timeline offset/.store in=\timelineoffset,
  timeline offset=0.05,
  initial week/.store in=\initialweek,
  initial week=1,
  end week/.store in=\endweek,
  end week=2,
  time point/.store in=\timepoint,
  time point=0.5,
  between day/.style args={#1 and #2 in #3}{% auxiliary style for days
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between week/.style args={#1 and #2 in #3}{% style for weeks
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between month/.style args={#1 and #2 in #3}{% auxiliary style for months
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  between year/.style args={#1 and #2 in #3}{% auxiliary style for years
    initial week=#1,
    end week=#2,
    time point=#3,
  },
  involvement degree/.store in=\involvdegree,
  involvement degree=2cm,
  phase color/.store in=\phasecol,
  phase color=red!50!orange,
  phase appearance/.style={
    circle,
    opacity=0.3,
    minimum size=\involvdegree,
    fill=\phasecol
  },
}
% settings to customize aspect of timeline
\newif\ifcustominterval
\pgfkeys{/tikz/timeline/.cd,
  custom interval/.is if=custominterval,
  custom interval=false,
}

% settings to deploy milestones
\pgfkeys{/tikz/milestone/.cd,
  at/.store in=\msstartpoint,
  at=phase-1.north,
  circle radius/.store in=\milestonecircleradius,
  circle radius=0.1cm,
  direction/.store in=\msdirection,
  direction=90:2cm,
  text/.store in=\mstext,
  text={},
  text options/.code={\tikzset{#1}},
}

\newcommand{\reftimespan}{\MakeLowerCase{\timespan}}

\newcommand{\timeline}[2][]{
  \pgfkeys{/tikz/timeline/.cd,#1}
  \draw[fill,opacity=0.8] (0,0) rectangle (\timelinewidth,\timelineheight);
  \shade[top color=black, bottom color=white,middle color=black!20]
    (0,0) rectangle (\timelinewidth,-\timelineoffset);
  \shade[top color=white, bottom color=black,middle color=black!20]  
    (0,\timelineheight) rectangle (\timelinewidth,\timelineheight+\timelineoffset);

  \ifcustominterval%
    \foreach \smitem [count=\tlmxi] in {#2}  {\global\let\maxsmitem\tlmxi}%
  \else%
    \foreach \smitem [count=\tlmxi] in {1,...,#2}  {\global\let\maxsmitem\tlmxi}%
  \fi%
  
  \pgfmathsetmacro\position{\timelinewidth/(\maxsmitem+1)}
  \node at (0,0.5\timelineheight)(\timespan-0){\phantom{Week 0}};
 
  \ifcustominterval%
    \foreach \x[count=\tlmxi] in {#2}{%
      \node[text=white,text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \else%
    \foreach \x[count=\tlmxi] in {1,...,#2}{%
      \node[text=white, text depth=0pt]at +(\tlmxi*\position,0.5\timelineheight) (\timespan-\tlmxi) {\timespan\ \x};%
    }%
  \fi%  
}

\newcounter{involv}
\setcounter{involv}{0}

\newcommand{\phase}[1]{
\stepcounter{involv}
\node[phase appearance,#1] 
 (phase-\theinvolv)
 at ($(\timespan-\initialweek)!\timepoint!(\timespan-\endweek)$){};
}

\newcommand{\initialphase}[1]{
\node[phase appearance,#1,anchor=west,between week=0 and 1 in 0,] 
 (phase-\theinvolv)
 at ($(\timespan-0)!0!(\timespan-1)$){};
\setcounter{involv}{0} 
}

\newenvironment{phases}{\begin{pgfonlayer}{background}}{\end{pgfonlayer}}

\newcommand{\addmilestone}[1]{
\pgfkeys{/tikz/milestone/.cd,#1}
\draw[double,fill] (\msstartpoint) circle [radius=\milestonecircleradius];
\draw(\msstartpoint)--++(\msdirection)node[/tikz/milestone/text options]{\mstext};
}

% HISTORY
% 0.1 -> initial release
% 0.2 -> customizable timespan label
% 0.3 -> \timeline command with custom intervals
%             styles ``between x''
%             removed unnecessary call to xstring
% 0.3a -> text depth for timeline labels
% 0.3b -> \xi conflict - thanks Enrico Gregorio (egreg) https://tex.stackexchange.com/q/476089
